Zooid: a DSL for Certified Multiparty Computation

We design and implement Zooid, a domain specific language for certified multiparty communication, embedded in Coq and implemented atop our mechanisation framework of asynchronous multiparty session types (the first of its kind). Zooid provides a fully mechanised metatheory for the semantics of global and local types, and a fully verified end-point process language that faithfully reflects the type-level behaviours and thus inherits the global types properties such as deadlock freedom, protocol compliance, and liveness guarantees.

==> conclusion.tex <==
\section{Conclusion and Future Work}\label{sec:conclusion}

In this work, we design and implement a certified language for
end-point processes supporting multiparty session types. We start by
mechanising the meta-theory of asynchronous MPST, and build \dslName,
a process language on top of that. Using code extraction, we interface
with OCaml code to produce running implementations of the processes
specified in \dslName.

% In this work, we formalise and mechanise %, for the first time,
% the metatheory of multiparty session types.
% To the best of our knowledge, this is a novelty itself,
% moreover it gave us the opportunity to explore new proof techniques for MPST: we add an intermediate asynchronous semantic representation for session types
%  based on coinductive trees and, building on this, we show that global types and the local types, obtained by their projection, produce equivalent execution traces.
% Second, we define a process calculus, together with its typing
% discipline and its LTS semantics. %based on labelled transition systems.
% We show that well-typed
% processes produce traces that are complete subtraces of their global
% type, to put it short: \emph{well-typed processes follow their global
%   types}.
%   Finally, we define \dslName{} as an embedded DSL to write
% intrinsically typed end-point processes. By building on top of the
% metatheory, \dslName{} programs are guaranteed to follow the expected
% traces of their global types. Ideally, the programmer would use \dslName{} to
% produce certified implementations of their chosen processes. Moreover,
% each process of the
% protocol can be specified independently, and in different languages, as long as
% they use a compatible transport. To that we have
% added one last practical feature to \dslName{}: we have enabled Coq code
% extraction to OCaml executable code.
%% This development was started with the
%% clear intention of showing that implementing metatheory in a proof
%% assistant is both important for the theoretical and practical aspects
%% of the concurrent behavioural types.
%This works novel approach to the proof and the \dslName
%language are witnesses of this.
%We finish the paper by showing examples of \dslName programs.

This work on mechanising MPST and \dslName is a founding stone, there are many
exciting opportunities for future work. On top of our framework,
we plan to explore new ideas and extensions of the theory of session
types. The immediate next step is to make the proofs extensible, for
example by allowing easy integration of custom merge strategies,
adding advanced features such as indexed dependent session
types~\cite{Castro:2019:DPU:3302515.3290342} or timed
specifications~\cite{BYY2014,BLY2015}. Moreover, we intend to
apply the work in this paper (and its extensions) to
implement a certified toolchain for the Scribble protocol description
language ({\url{http://www.scribble.org}), also known as ``the practical
incarnation of multiparty session types''
\cite{10.1007/978-3-642-19056-8_4,FeatherweightScribble}. To this aim we plan to
translate from Scribble to MPST style global types, following the Featherweight
Scribble formalisation~\cite{FeatherweightScribble}.

%% Local Variables:
%% mode: latex
%% TeX-master: "main"
%% End:


==> related.tex <==
\section{Related Work} \label{sec:related}
In the concurrency and
behavioural types communities, there is growing interest in
mechanisation and the use of proof assistants to validate research.
Recent examples of this fact are two workshops, most recently the
Verification of Session Types~\cite{VEST:2020}, an online workshop to
present work on mechanisation efforts for session type system, and a
half day session on mechanical proofs and behavioural types, the BeHAPI
Workshop at ETAPS 2019~\cite{BeHAPI:2019}. These workshops provided a
venue to show relevant ongoing or already published work.
One such case is~\Citet{GTV20} that explores the interaction between
duality and recursive types, a delicate subject and how they take
advantage of mechanisation to formalise some of their results.
\citet{Krebbers:2020} explore the notion of semantic typing using a
concurrent separation logic as a semantic domain to explore reasoning
about process with channels typed by binary session types. Other
projects explore ways to build foundations to support further
development, such as mechanising the metatheory of the linear
$\pi$-calculus~\cite{Zalakian:2020}.

The scope and ambition of mechanisation is increasing and
collaborative projects that explore the space of available solutions
are an important tool for the community,
%, as exemplified
%by~\cite{Ravara:2020, diGiusto:2020, Peters:2020}
where they explore
different representations of binders (names, de~Bruijn indices/levels,
nominals respectively), see \citeN[Discussion]{VEST:2020}.
%% Other works explore options such as locally
%% nameless~\cite{Castro:2020}, and intrinsically typed representation
%% with support for linearity~\cite{Kokke:2019}.
%The question of binder
%representation is being explored from multiple points of view,
In this
work we sidetrack the question by designing \dslName to use a shallow
embedding of its binders (thus avoiding to need an explicit
representation for variables). In our experience, this is a simple and
valuable technique for the situations where it is applicable.

Other works also explore ideas on \emph{binary}
session types using proof assistants
and mechanised proofs. For example, \citet{Thiemann:2019} develops an
intrinsically typed semantics in Agda that provides preservation and a
notion of progress for binary session types. Additionally,
\citet{Tassarotti:2017} shows the correctness (in the Coq proof
assistant) of a compiler that uses an intermediate language based on a
simplified version of the GV system~\cite{Gay:2010} to add session types
to a functional programming language. And \citet{Orchard:2016}
discuss the relation between session types and effect systems, and
implement their code in the Agda proof assistant. Their
formalisation concentrates on translating between effect systems and
session types in a type preserving manner.
\citet{emtst:2019} present a type preservation of binary session
type~\cite{Honda:1998, Yoshida:2007} as a case study of using their
tool~\cite{Castro:2020}. Furthermore, \citet{Goto:2016} present a
session types system with session polymorphism and use Coq to prove
type soundness of their system.
Note that none of the above work on session types treats
\emph{multiparty session types} -- they are limited to
\emph{binary} session types.

%% The concurrency community is hard at work on reaping the value
%% of fully mechanised proofs, witnessed by the amount of
%% work done and onging work
%% on this subject.
Our work on MPST uses mechanisation to both give
a fresh look at
trace equivalence~\cite{DenielouYoshida2013} in MPST and to further
explore its relation to a process calculus. At the same time our aim
is to provide a bedrock for future projects dealing with the MPST
theories. And crucially, this is the first work that tackles
\emph{a full syntax of asynchronous multiparty session types}
that type the whole interaction as opposed to
binary session types that only type individual channels.

Regarding the choice of tool and inspiration in this work, we point
out that the first objective is to mechanise trace equivalence
between global and local types.  However, following a different
approach, one that suits the Coq proof assistant, our tool of choice.
For that, we took inspiration of more semantic representations of
session types~\cite{GHILEZAN2019127, Li-yao:2019}.
The choice of the Coq proof assistant~\cite{CoqManual} was
motivated by its stability, rich support for coinduction, and good
support for the extraction of certified code. Stability is important
since this is a codebase that we expect to work on and expand for
future projects. The proofs take advantage of small scale
reflection~\cite{Gonthier:2010} using Ssreflect to structure our
development. And given the pervasive need for greatest fixed points in
MPST, we extensively use the PaCo library~\cite{paco} for the proofs
that depend on coinduction.

%% Local Variables:
%% mode: latex
%% TeX-master: "main"
%% End:

